Learning-Augmented Query Policies for Minimum Spanning Tree with Uncertainty

We study how to utilize (possibly erroneous) predictions in a model for computing under uncertainty in which an algorithm can query unknown data. Our aim is to minimize the number of queries needed to solve the minimum spanning tree problem, a fundamental combinatorial optimization problem that has been central also to the research area of explorable uncertainty. For all integral $\gamma\ge 2$, we present algorithms that are $\gamma$-robust and $(1+\frac{1}{\gamma})$-consistent, meaning that they use at most $\gamma OPT$ queries if the predictions are arbitrarily wrong and at most $(1+\frac{1}{\gamma})OPT$ queries if the predictions are correct, where $OPT$ is the optimal number of queries for the given instance. Moreover, we show that this trade-off is best possible. Furthermore, we argue that a suitably defined hop distance is a useful measure for the amount of prediction error and design algorithms with performance guarantees that degrade smoothly with the hop distance. We also show that the predictions are PAC-learnable in our model. Our results demonstrate that untrusted predictions can circumvent the known lower bound of~$2$, without any degradation of the worst-case ratio. To obtain our results, we provide new structural insights for the minimum spanning tree problem that might be useful in the context of query-based algorithms regardless of predictions. In particular, we generalize the concept of witness sets -- the key to lower-bounding the optimum -- by proposing novel global witness set structures and completely new ways of adaptively using those.

==> input-prelim-short.tex <==
%\paragraph*{Problem definition}
\subparagraph*{Problem definition}
In the {\em minimum spanning tree (MST) problem under \nnew{explorable} uncertainty}, we are given a graph $G=(V,E)$, with uncertainty intervals $I_e$ %, i.e., $I_e = (L_e,U_e)$ or $I_e = [w_e]$, 
and predicted values $\pred{w}_e \in I_e$ for the weight of each edge $e \in E$.
The \emph{true} value of interval $I_e$ is denoted by $w_e$ and can be revealed by a \emph{query}.
%A minimum spanning tree (MST) 
\nnew{An MST} is a tree that connects all vertices of $G$ at a minimum total edge weight.
The task is to find an MST with respect to the true values~$w_e$. %of the edge weights.

The goal is to solve the task using a minimum number of queries. 
Note that the exact value of a solution, i.e., the weight of the MST, does not need to be determined. \nnew{We may assume w.l.o.g.\ that the given graph $G$ is biconnected.} 
We further assume that each uncertainty interval is either open or trivial, i.e., $I_i = (L_i,U_i)$ or $I_i = \{w_i\}$; \nnew{a standard technical assumption to avoid a simple lower bound of \nnew{$|E|$}  
on the competitive ratio \cite{gupta16queryselection,erlebach08steiner_uncertainty}}.
%as otherwise a simple lower bound of \nnew{$|E|$}  
%on the competitive ratio exists (as shown in \cite{gupta16queryselection}
%for the minimum problem with uncertainty, which translates directly to the maximum problem and hence
%to the MST problem in a graph that is a single cycle).

%Further,
We study \emph{adaptive %\nic{Added line break which should make the adaptivity paragraph more visible.} 
strategies} that make queries sequentially and utilize the results of previous steps to decide upon the next query.
We impose no time/space complexity constraints on the algorithms, as we are interested in understanding the competitive ratio of the problems.
%We assume the algorithms never query intervals that are trivial or that were previously queried. % already.
%A set $W$ of queries is called a \emph{witness set} \cite{bruce05uncertainty,erlebach08steiner_uncertainty} if every feasible solution (i.e., every set of queries that solves the problem) contains at least one query in~$W$.

\subparagraph*{Competitive analysis}
We %employ competitive analysis and 
compare the outcome of our algorithms with the best offline solution, i.e., the minimum number of queries needed to verify a solution when all values are known in advance. We call the offline variant of our problem \emph{verification problem}.
{By $\OPT$ we denote an arbitrary optimal query set for the verification problem %, and by $\opt$ its cardinality. For an algorithm for the online problem, we denote 
and by $\ALG$ the set of queries that an algorithm makes.\nic{cardinality is clear, removed}  % and by $|\ALG|$ the cardinality of that set.}
%\mur{Maybe we can eliminate $\ALG$ and $|\ALG|$.}
%\nic{heavily used in MST}
An algorithm is $\rho$-{\em competitive} if it executes, for any problem instance, at most $\rho \cdot {\opt}$ queries.
%, where $Q^*$ is an optimal query set of the verification problem. 
%
Further, we quantify the performance of our algorithms depending on the quality of predictions. For the extreme cases, we say that an algorithm is $\alpha$-\emph{consistent} if it is $\alpha$-competitive if the predictions are correct, and $\beta$-\emph{robust} if it is $\beta$-competitive if the predictions are inaccurate. 

\nic{MARKER for overview} Clearly, an algorithm that assumes the predicted values to be correct, solves the verification problem, and makes queries accordingly is $1$-consistent. However, such an algorithm may have an arbitrarily bad performance if the predictions are incorrect. Similarly, the known deterministic $2$-competitive algorithm for the online MST problem without predictions~\cite{erlebach08steiner_uncertainty} is $2$-robust and $2$-consistent. The known lower bound of $2$ rules out any robustness factor less than $2$ for our model.  {It builds on the following simple example with two intersecting intervals $I_a,I_b$ that are candidates for the largest edge weight in a cycle. No matter which interval a deterministic algorithm queries first, say $I_a$, the realized value could be $w_a\in I_a\cap I_b$, which requires a second query. If the adversary chooses $w_b\notin I_a\cap I_b$, querying just $I_b$ would have been sufficient to identify the interval with larger true value.} 

%We give a bound on the best~achievable~tradeoff between consistency and robustness. Later, we will provide algorithms with matching performance guarantees.\nic{shall we move this behind the upper bound to confirm that it is tight? But then, what about Thm. 2?}\tom{Stating theorems inside a section on definitions seems a bit strange?}
%
%\begin{restatable}{theorem}{ThmLBTradeoffWithoutError}
%%\begin{theorem}
%\label{theo_minimum_combined_lb}
%  Let %$\beta \in \ZZ$ with 
%  $\beta \geq 2$ be a fixed integer.
%  For the MST problem under uncertainty, there is no deterministic $\beta$-robust algorithm that is $\alpha$-consistent for $\alpha < 1 + \frac{1}{\beta}$. And vice versa, no deterministic $\alpha$-consistent algorithm, with $\alpha>1$, is $\beta$-robust for $\beta < \max\{\frac{1}{\alpha-1},2\}$.
%%\end{theorem}
%\end{restatable}
%
%\begin{proof}
%We state the proof for the minimum problem. It can be easily adapted to the other two; {for the MST consider a single cycle.} 
%Consider the instance in Figure~\ref{fig_combined_lb_min_single_set} with $\beta+1$ intervals and a single set.
%If the predicted values are correct, then any feasible solution must query $I_{1}, \ldots, I_{\beta}$.
%%
%Suppose there is a $\beta$-robust and $\alpha$-consistent algorithm with $\alpha=1 + \frac{1}{\beta}-\eps$ for some $\eps>0$. 
%It must query $I_{1}, \ldots, I_{\beta}$ first, as otherwise, it would query $\beta+1$ intervals while there is an optimal query set of size $\beta$, in case all predictions are correct.  
%Suppose w.l.o.g.\ that the algorithm queries intervals in order of increasing indices. Consider the choice $w_i = \pred{w}_i$, for $i = 1, \ldots, \beta - 1$, and then $w_{\beta} \in I_0$ and $w_0 \notin I_1 \cup \ldots \cup I_{\beta}$.
%This forces the algorithm to query also~$I_0$, while an optimal solution only queries~$I_0$.
%Thus any such algorithm has robustness at least~$\beta+1$, a contradiction.
%\end{proof}

%For each of the considered problems, we give an algorithm that achieves the best possible consistency-robustness tradeoff. \nic{Need to be careful and check at the end.}

%\begin{figure}[tb]
%  \centering
%  \subfigure[]{\label{fig_combined_lb_min_single_set}
%  \begin{tikzpicture}[line width = 0.3mm, scale=0.8]
%    \intervalpr{$I_1$}{1}{3}{0}{2.5}{2.5}
%    \intervalpr{$I_2$}{1}{3}{0.5}{2.5}{2.5}
%    \intervalpr{$I_\beta$}{1}{3}{1.5}{2.5}{1.5}
%    \path (2, 0.5) -- (2, 1.6) node[font=\normalsize, midway, sloped]{$\dots$};
%
%    \intervalpr{$I_0$}{0}{2}{-0.5}{1.5}{0.5}
%  \end{tikzpicture}}\quad
%  \subfigure[]{\label{fig_lb_wrong_predictions}
%  \begin{tikzpicture}[line width = 0.3mm, scale=0.8]
%    \intervalpr{$I_1$}{0}{2}{0}{0.5}{0.5}
%    \intervalpr{$I_2$}{0}{2}{0.5}{0.5}{0.5}
%    \intervalpr{$I_n$}{0}{2}{1.5}{0.5}{1.5}
%    \path (1, 0.5) -- (1, 1.6) node[font=\normalsize, midway, sloped]{$\dots$};
%
%    \intervalpr{$I_{n+1}$}{1}{3}{2}{2.5}{2.5}
%    \intervalpr{$I_{n+2}$}{1}{3}{2.5}{2.5}{2.5}
%    \intervalpr{$I_{2n}$}{1}{3}{3.5}{2.5}{2.5}
%    \path (2, 2.5) -- (2, 3.6) node[font=\normalsize, midway, sloped]{$\dots$};
%  \end{tikzpicture}}\quad
%  \subfigure[]{\label{fig_lb_error_measure}
%  \begin{tikzpicture}[line width = 0.3mm, scale=0.8]
%    \intervalpr{$I_1$}{0}{2}{0}{1.5}{1.5}
%    \intervalpr{$I_2$}{1}{3}{0.5}{1.5}{2.5}
%  \end{tikzpicture}}
%   \caption{Instances for lower bounds.
%  Red crosses indicate predicted values, and green circles show correct values.
%  \subref{fig_combined_lb_min_single_set}~Lower bound on robustness-consistency tradeoff.
%  \subref{fig_lb_wrong_predictions} Lower bound based on the number of inaccurate predictions.
%  \subref{fig_lb_error_measure}~Lower bound based on error measures.
%  \label{fig_lowerbounds}
%  }
%\end{figure}


\subparagraph*{Accuracy of predictions $-$ hop distance}
We aim for a more fine-grained performance analysis giving guarantees that depend on the quality of predictions. %To that end,
A very natural, simple error measure is the number of inaccurate predictions $k_\#=|\{e \in E\,|\, w_e \not= \w_e\}|$. However, we can show that even for $k_{\#} \geq 1$\tom{Should we replace `even for $k_{\#}\ge 1$' by `even for $k_{\#}=1$'?} the competitive ratio cannot be better than the known lower bound of~$2$ \tomc{(see Lemma~\ref{lem:lb_wrong_predictions} in Appendix~\ref{app:prelim} for a proof)}.
the interleaving  structure of intervals. Similarly, using an $L_1$ error metric such as
$\sum_{e\in E}|w_e - \w_e|$ would not be meaningful because only
the \emph{order} of the values and the interval endpoints matters for our problems.
To address this, we consider a refined measure for the prediction quality.

\jnew{If we consider only a single predicted value $\w_e$ for some $e \in E$, then, in a sense, this value predicts the relation of the true value $w_e$ to the intervals of edges $e' \in E\setminus \{e\}$.\jen{Proposal for an alternative hop distance definition. This counts $w_e \le L_{e'} < U_{e'} \le \w_e$ only as a single error, but I think this is consistent with our proofs.}
In particular, w.r.t.~a fixed $e' \in E\setminus \{e\}$, the value $\w_e$ predicts whether $w_e$ is left of $I_{e'}$ ($\w_e \le L_{e'}$), right of $I_{e'}$ ($\w_e \ge U_{e'}$), or contained in $I_{e'}$ ($L_{e'} < \w_e < U_{e'}$).
Interpreting the prediction $\w_e$ in this way, the prediction is \enquote{wrong} (w.r.t.~a fixed $e' \in E\setminus \{e\}$) if the predicted relation of the true value $w_e$ to interval $I_{e'}$ is not actually true, e.g., $w_e$ is predicted to be left of $I_{e'}$ ($\w_e \le L_{e'}$) but the actual $w_e$ is either contained in or right of $I_{e'}$ ($w_e > L_{e'}$).
Formally, we define the function $\jo_{e'}(e)$ that indicates whether the predicted relation of $w_e$ to $I_{e'}$ is true ($\jo_{e'}(e) = 0$) or not ($\jo_{e'}(e) = 1$).
With the prediction error $\jo(e)$ for a single $e \in E$, we want to capture the number of relations between $w_e$ and intervals $I_{e'}$ with $e' \in E\setminus \{e\}$ that are not accurately predicted.
Thus, we define $\jo(e) = \sum_{e' \in E\setminus \{e\}} \jo_{e'}(e)$.
For a set of edges $E' \subseteq E$, we define $\jo(E') = \sum_{e \in E'} \jo(e)$.
Consequently, with the error for the complete instance we want to capture the total number of wrongly predicted relations and, therefore, define it by $\jo_h=\jo(E)$.
We call this error measure $\jo_h$ the {\em hop distance}.

Symmetrically, we can define $\oj(e) = \sum_{e' \in E\setminus \{e\}} \jo_{e}(e')$ and $\jo(E') = \sum_{e \in E'} \oj(e)$ for subset $E' \subseteq E$. 
Then $\jo(E) = \jo_h = \oj(E)$ follows by reordering the summations. 
}


%%\paragraph{Hop distance} 
%% \emph{Hop distance.} 
%The {\em hop distance},\nic{discuss: how to rewrite (intuitive + correct)} which we define below, captures naturally the relation between a predicted and a true value in relation to other intervals.
%For a non-trivial interval $I_e=(L_e,U_e)$,
%we say that the value of interval $I_{e'}$ \emph{passes over} $L_e$ if one of $w_{e'},\w_{e'}$ is
%$\le L_e$ and the other is $>L_e$. Similarly,
%the value of $I_{e'}$ \emph{passes over} $U_e$ if one of $w_{e'},\w_{e'}$ is
%$< U_e$ and the other is $\ge U_e$. Intuitively, the value of $I_{e'}$ passes over one endpoint of~$I_e$
%if it enters or leaves $I_{e}$, and it passes over both endpoints of $I_e$ if it jumps over $I_e$
%when going from predicted to true values.
%For a trivial interval $I_e=\{w_e\}$, we say that the value of $I_{e'}$
%%\emph{moves to/from} $I_j$ if exactly one of $w_i,\w_i$ is equal to $w_j$, and we say that the value of $I_i$
%\emph{jumps over}~$I_e$ if one of $w_{e'},\w_{e'}$ is strictly smaller than $w_j$ and the other is strictly
%larger than $w_e$.
%{To avoid counting values passing over endpoints of irrelevant intervals,} 
%let $A_e$ be the set of intervals that potentially interact with $I_e$. % (defined in a problem-specific
%%way).
%When considering the MST problem, we consider the maximal biconnected component containing $e$, i.e., $A_e$
%is the set of all intervals on cycles containing~$e$.
%Now define $\jo(e')$ to be the number of non-trivial intervals $I_{e}\in A_{e'}$ such that the value of~$I_{e'}$ passes
%over $L_e$ plus the number of non-trivial intervals $I_{e}\in A_{e'}$ such that the value of~$I_{e'}$ passes
%over $U_e$, plus the number of trivial intervals $I_e=\{w_e\}$ in $A_{e'}$ such that
%the value of $I_{e'}$ jumps over~$I_e$.
%For a subset of edges $E' \subseteq E$, let $\jo(E') = \sum_{e \in E'} \jo(e)$.
%The hop distance of a given instance is then $k_h = \jo(E)$; 
%{see also Figure~\ref{fig_error_ex}}. % for an example.}


%\red{Alternatively, let $\oj(e)$ with $e \in E$ be the number of edges $e'$ such that the value of $e'$ passes over an endpoint of $I_e$.
%For a subset $U \subseteq E$, let $\oj(U) = \sum_{e \in U} \oj(e)$.
%Note that $k_h = \oj(E)$ holds by reordering summations.\todo{TODO: $\oj$ un $\jo$ aneinander anpassen. Leider brauchen wir beides.}
%}


Note that $k_{\#} = 0$ implies $k_h = 0$, so Theorem~\ref{theo_minimum_combined_lb} implies that no algorithm can simultaneously have competitive ratio better than $1 + \frac{1}{\beta}$ if $k_h = 0$ and $\beta$ for arbitrary~$k_h$.

\jnew{In~\Cref{app:learning} we show that the predictions are indeed PAC learnable w.r.t.~$k_h$.}

\begin{theorem}
\label{thm:learning}
\jnew{The predicted values $\pred{w}$ for a given instance of MST under explorable uncertainty are PAC learnable w.r.t.~$k_h$ with polynomial time and sample complexity.}
\end{theorem}

\begin{figure}[t]
	\centering
	\begin{subfigure}[l]{0.35\textwidth}
	add a cycle?	
	\end{subfigure}
	\hspace*{1cm}
	\begin{subfigure}[r]{0.35\textwidth}
		\begin{tikzpicture}[line width = 0.3mm, scale = 0.9, transform shape]	
		\intervalpr{$I_1$}{0}{4}{1.5}{1}{2.75}	
		\intervalpr{$I_2$}{1.5}{6}{2.25}{4.5}{2}	
		\intervalpr{$I_3$}{2.5}{6}{3}{4.5}{5.5}							
		\intervalpr{$I_4$}{3}{6}{3.75}{3.25}{3.75}		
		
		\begin{scope}[on background layer]
		\draw[line width = 0.2mm,,lightgray] (0,1) -- (0,4);
		\draw[line width = 0.2mm,,lightgray] (1.5,1) -- (1.5,4);
		\draw[line width = 0.2mm,,lightgray] (2.5,1) -- (2.5,4);
		\draw[line width = 0.2mm,,lightgray] (3,1) -- (3,4);
		\draw[line width = 0.2mm,,lightgray] (6,1) -- (6,4);
		\draw[line width = 0.2mm,,lightgray] (4,1) -- (4,4);
		\end{scope}
		
		\draw[decoration= {brace, amplitude = 5 pt, aspect = 0.5}, decorate] (2.75,1.3) -- (1,1.3);
		\node[] (l1) at (1.85,1) {\scalebox{0.75}{$h_1=2$}};
		
		\draw[decoration= {brace, amplitude = 5 pt, aspect = 0.5}, decorate] (4.5,2.1) -- (2,2.1);
		\node[] (l1) at (3.2,1.8) {\scalebox{0.75}{$h_2=3$}};
		
		\draw[decoration= {brace, amplitude = 2.5 pt, aspect = 0.5}, decorate] (5.5,2.85) -- (4.5,2.85);
		\node[] (l1) at (4.95,2.6) {\scalebox{0.75}{$h_3=0$}};
		
		\draw[decoration= {brace, amplitude = 1 pt, aspect = 0.5}, decorate] (3.75,3.6) -- (3.25,3.6);
		\node[] (l1) at (3.5,3.4) {\scalebox{0.75}{$h_4=0$}};
		\end{tikzpicture}
	\end{subfigure}
%	\hspace*{2cm}
%	\begin{subfigure}[r]{0.35\textwidth}
%	\begin{tikzpicture}[line width = 0.3mm, scale = 0.9, transform shape]
%		\intervalpr{$I_1$}{0}{4}{1.5}{1}{1}		
%		\intervalpr{$I_2$}{1.5}{6}{2.25}{3.25}{5.5}		
%		\intervalpr{$I_3$}{2.5}{6}{3}{3.25}{5.5}								
%		\intervalpr{$I_4$}{3}{6}{3.75}{3.25}{5.5}				
%		
%		% Dummy for spacing:
%		\node[] (l1) at (1.85,0.95) {};	
%		\end{tikzpicture}
%	\end{subfigure}
\caption{
 Example of a single cycle with uncertain edge weights from intersecting intervals  %set $S=\{I_1,I_2,I_3,I_4\}$. 
$I_1,I_2,I_3,I_4$. Circles illustrate true values and crosses illustrate the predicted values. %\subref{fig_hop_ex} 
%Predictions and true values with 
The total hop distance is $k_h = 5$.
%\subref{fig_man_ex} Predictions and true values with a mandatory query distance of $k_M = 1$.
}
\label{fig_error_ex}
\end{figure}


